Corner asymptotics of the magnetic potential in the eddy-current model

In this paper, we describe the magnetic potential in the vicinity of a corner of a conducting body embedded in a dielectric medium in a bidimensional setting. We make explicit the corner asymptotic expansion for this potential as the distance to the corner goes to zero. This expansion involves singular functions and singular coefficients. We introduce a method for the calculation of the singular functions near the corner and we provide two methods to compute the singular coefficients: the method of moments and the method of quasi-dual singular functions. Estimates for the convergence of both approximate methods are proven. We eventually illustrate the theoretical results with finite element computations. The specific non-standard feature of this problem lies in the structure of its singular functions: They have the form of series whose first terms are harmonic polynomials and further terms are genuine non-smooth functions generated by the piecewise constant zeroth order term of the operator.

==> figures/Mac-LXXX-w45 <==

#set terminal windows
#set terminal x11
#set terminal postscript eps enhanced monochrome
#set terminal postscript eps enhanced color


#set terminal postscript eps enhanced color "Times-Roman" 22
#set terminal postscript eps enhanced monochrome "Times-Roman" 18

set terminal postscript eps enhanced color "Times-Roman" 20
set terminal postscript eps enhanced color "Times-Roman" 18

set yrange [*:*]

set size ratio 0.618
set size ratio 0.5
#set size noratio

# --------------------------------------------
# --------------------------------------------

set grid

#set nolabel
#set label "h-form., 50 Hz" at 2200, 2.45*2

fy = 1
fx = 1

set angles radians

#####################################################
# 
#####################################################

##########
set output 'F-L00-w45.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/4)"
set ylabel "|{/Symbol {L}}^{0, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Imaginary part" at 6e-5, 4e-4
set label  "Real part" at 2e-4, 2.5e-5
set label  "Real part" at 1.4e-4, 3e-7
set label  "Imaginary part" at 1.75e-4, 2e-9

set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar = 0.1144499045465204
ai = -0.04649073357253156

plot [5e-5:0.005]\
     'L001_w45.txt' u 1:(abs($2-ar)) notitle w lp lt 1 pt 1 lw 2, \
     'L001_w45.txt' u 1:(abs($3-ai)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/2e13 title 'O(R_0^4 log R)' lt 3, \
     'L000_w45.txt' u 1:(abs($2-ar)) notitle w lp lt 1 pt 1 lw 2, \
     'L000_w45.txt' u 1:(abs($3-ai)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**2/1.7e7 title 'O(R_0^2 log R)' lt 4

#plot [5e-5:0.005]\
#     'L000_w45.txt' u 1:(abs($2-ar)) title 'k^{0, 0}, n = 0 (no shadow)' w lp lw 2, \
#     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**2/1.7e7 title 'O(R_0^2 log R)', \
#     'L001_w45.txt' u 1:(abs($2-ar)) title 'k^{0, 0}, n = 1 (shadow)' w lp lw 2, \
#     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/1.5e13 title 'O(R_0^4 log R)', \
#     'L000_w45.txt' u 1:(abs($3-ai)) title 'k^{0, 0}, n = 0 (no shadow)' w lp lw 2, \
#     'L001_w45.txt' u 1:(abs($3-ai)) title 'k^{0, 0}, n = 1 (shadow)' w lp lw 2


#pause -1

set nokey

##########
set output 'F-L10-w45.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/4)"
set ylabel "|{/Symbol {L}}^{1, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 1.9e-4, 2.8e-3
set label  "Imaginary part" at 4e-4, 3e-4

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar1 = -12.970662352159
ai1 = -5.4091591736398

plot [8e-5:0.005]\
     'L101_w45.txt' u 1:(abs($2-ar1)) notitle w lp lt 1 pt 1 lw 2, \
     'L101_w45.txt' u 1:(abs($3-ai1)) notitle w lp lt 2 pt 2 lw 2, \
     (zeta*x*(1+(abs(log(x)))**0.5))**4/x/1.5e12 title 'O(R_0^4 R^{-1})' lt 3

#pause -1

set nokey

##########


##########
set output 'F-L20-w45.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/4)"
set ylabel "|{/Symbol {L}}^{2, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 1.9e-4, 3.5e1
set label  "Imaginary part" at 4e-4, 3e0

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar2 = 1406.17543172
ai2 = 4599.1999943653

plot [8e-5:0.005]\
     'L201_w45.txt' u 1:(abs($2-ar2)) notitle w lp lt 1 pt 1 lw 2, \
     'L201_w45.txt' u 1:(abs($3-ai2)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/x**2/2.5e12 title 'O(R_0^4 R^{-2} log R)' lt 3

#pause -1

set nokey

##########


##########
set output 'F-L30-w45.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/4)"
set ylabel "|{/Symbol {L}}^{3, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 2.3e-4, 1.5e4
set label  "Imaginary part" at 4e-4, 2e3

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar3 = 93044.907016993
ai3 = -154837.94059187

plot [8e-5:0.005]\
     'L301_w45.txt' u 1:(abs($2-ar3)) notitle w lp lt 1 pt 1 lw 2, \
     'L301_w45.txt' u 1:(abs($3-ai3)) notitle w lp lt 2 pt 2 lw 2, \
     (zeta*x*(1+(abs(log(x)))**0.5))**4/x**3/1.7e12 title 'O(R_0^4 R^{-3})' lt 3

#pause -1

set nokey

##########


#plot x*x


set xrange [*:*]
set yrange [*:*]

#set terminal x11
#set terminal windows


==> figures/Mac-LXXX-w90 <==

#set terminal windows
#set terminal x11
#set terminal postscript eps enhanced monochrome
#set terminal postscript eps enhanced color


#set terminal postscript eps enhanced color "Times-Roman" 22
#set terminal postscript eps enhanced monochrome "Times-Roman" 18

set terminal postscript eps enhanced color "Times-Roman" 20
set terminal postscript eps enhanced color "Times-Roman" 18

set yrange [*:*]

set size ratio 0.618
set size ratio 0.5
#set size noratio

# --------------------------------------------
# --------------------------------------------

set grid

#set nolabel
#set label "h-form., 50 Hz" at 2200, 2.45*2

fy = 1
fx = 1

set angles radians

#####################################################
# 
#####################################################

##########
set output 'F-L00-w90.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/2)"
set ylabel "|{/Symbol {L}}^{0, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Imaginary part" at 6e-5, 4e-4
set label  "Real part" at 2e-4, 2.5e-5
set label  "Real part" at 1.4e-4, 3e-7
set label  "Imaginary part" at 3.5e-4, 2e-9

set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar = 0.07672291744995079
ai = -0.03979502102718694

plot [5e-5:0.005]\
     'L001_w90.txt' u 1:(abs($2-ar)) notitle w lp lt 1 pt 1 lw 2, \
     'L001_w90.txt' u 1:(abs($3-ai)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/2e13 title 'O(R_0^4 log R)' lt 3, \
     'L000_w90.txt' u 1:(abs($2-ar)) notitle w lp lt 1 pt 1 lw 2, \
     'L000_w90.txt' u 1:(abs($3-ai)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**2/1.7e7 title 'O(R_0^2 log R)' lt 4

#plot [5e-5:0.005]\
#     'L000_w90.txt' u 1:(abs($2-ar)) title 'k^{0, 0}, n = 0 (no shadow)' w lp lw 2, \
#     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**2/1.7e7 title 'O(R_0^2 log R)', \
#     'L001_w90.txt' u 1:(abs($2-ar)) title 'k^{0, 0}, n = 1 (shadow)' w lp lw 2, \
#     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/1.5e13 title 'O(R_0^4 log R)', \
#     'L000_w90.txt' u 1:(abs($3-ai)) title 'k^{0, 0}, n = 0 (no shadow)' w lp lw 2, \
#     'L001_w90.txt' u 1:(abs($3-ai)) title 'k^{0, 0}, n = 1 (shadow)' w lp lw 2


#pause -1

set nokey

##########
set output 'F-L10-w90.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/2)"
set ylabel "|{/Symbol {L}}^{1, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 1.9e-4, 3.2e-3
set label  "Imaginary part" at 4e-4, 3.5e-4

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar1 = -14.606261861557
ai1 = -4.6847066396195

plot [8e-5:0.005]\
     'L101_w90.txt' u 1:(abs($2-ar1)) notitle w lp lt 1 pt 1 lw 2, \
     'L101_w90.txt' u 1:(abs($3-ai1)) notitle w lp lt 2 pt 2 lw 2, \
     (zeta*x*(1+(abs(log(x)))**0.5))**4/x/1.5e12 title 'O(R_0^4 R^{-1})' lt 3

#pause -1

set nokey

##########


##########
set output 'F-L20-w90.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/2)"
set ylabel "|{/Symbol {L}}^{2, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 1.9e-4, 3.5e1
set label  "Imaginary part" at 4e-4, 5e0

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar2 = 1186.4404661845
ai2 = 3243.1380300909

plot [8e-5:0.005]\
     'L201_w90.txt' u 1:(abs($2-ar2)) notitle w lp lt 1 pt 1 lw 2, \
     'L201_w90.txt' u 1:(abs($3-ai2)) notitle w lp lt 2 pt 2 lw 2, \
     -log(x)*(zeta*x*(1+(abs(log(x)))**0.5))**4/x**2/2.5e12 title 'O(R_0^4 R^{-2} log R)' lt 3

#pause -1

set nokey

##########


##########
set output 'F-L30-w90.eps'
set xrange [*:*]

#set key top right Left reverse width -24

set key bottom right box
#set key 44,0.32,0
set key nobox
set xlabel "r (m) ({/Symbol {d}} = 0.005 m, {/Symbol {w}} = {/Symbol {p}}/2)"
set ylabel "|{/Symbol {L}}^{3, 0} - A_{FEM, corner}| (Wb/m)"

fx = 1
fy = 1
set xrange [*:*]
set yrange [*:*]
set xrange [*:*]
set yrange [*:*]

set logscale x
set logscale y

#set ytics 100

set nolabel
set label  "Real part" at 2.3e-4, 1.5e4
set label  "Imaginary part" at 4e-4, 3e3

#set label  "k^{0, 0}, n = 0 (no shadow)" at 1.3e-4, 4e-3
#set label  "k^{0, 0}, n = 1 (shadow)" at 7e-4, 3e-7


mu0 = 4.e-7 * pi
sigma_Cond = 1.e7
mur_Cond = 1

delta_fixed = 5.e-3

Freq = 2./delta_fixed**2 / (2.*pi*sigma_Cond*mur_Cond*mu0)

zeta = 2.*pi*Freq*mu0*sigma_Cond/4.

ar3 = 59880.403659582
ai3 = -110272.12514389

plot [8e-5:0.005]\
     'L301_w90.txt' u 1:(abs($2-ar3)) notitle w lp lt 1 pt 1 lw 2, \
     'L301_w90.txt' u 1:(abs($3-ai3)) notitle w lp lt 2 pt 2 lw 2, \
     (zeta*x*(1+(abs(log(x)))**0.5))**4/x**3/1.7e12 title 'O(R_0^4 R^{-3})' lt 3

#pause -1

set nokey

##########


#plot x*x


set xrange [*:*]
set yrange [*:*]

#set terminal x11
#set terminal windows

